Fast Kinodynamic Planning on the Constraint Manifold with Deep Neural Networks

Motion planning is a mature area of research in robotics with many well-established methods based on optimization or sampling the state space, suitable for solving kinematic motion planning. However, when dynamic motions under constraints are needed and computation time is limited, fast kinodynamic planning on the constraint manifold is indispensable. In recent years, learning-based solutions have become alternatives to classical approaches, but they still lack comprehensive handling of complex constraints, such as planning on a lower-dimensional manifold of the task space while considering the robot's dynamics. This paper introduces a novel learning-to-plan framework that exploits the concept of constraint manifold, including dynamics, and neural planning methods. Our approach generates plans satisfying an arbitrary set of constraints and computes them in a short constant time, namely the inference time of a neural network. This allows the robot to plan and replan reactively, making our approach suitable for dynamic environments. We validate our approach on two simulated tasks and in a demanding real-world scenario, where we use a Kuka LBR Iiwa 14 robotic arm to perform the hitting movement in robotic Air Hockey.

==> backup.tex <==
\subsection{Backup}

\subsubsection{Observations}
Piotr's observations:
\begin{enumerate}
    \item From the beginning of learning $\nabla\Loss_{\ddq} \approx 10^3 \nabla\Loss_{\dq} \approx 10^3 \Loss_{\FK} \approx   10^3\nabla t$
    \item If we start with all $\alpha_{\cdot} = 0$, then time of the movement $t$ explodes and after some time it is brought down, however, then short movements last unreasonably long
    \item If we start with very small learning rate like $10^{-7}$ then configurations are trained to optimize everything as well as possible, but the time is not being optimized at all for some time, and then it goes unreasonably high
    \item If we set initial values for $\alpha_{\cdot}$ such that we will equalize the impact of different gradients, then it seems to work, but after initially good training the time also goes up 
    \item It seems that the time B-spline is in these cases wrongly optimized, the resultant $\rate^{-1}$ should be pumped up at the beginning and end of the movement (where the violations of the acceleration constraint are the biggest (it stems from the way we construct the B-splines, especially the knot vector)), however it is scaled up for all values of $s$ instead
\end{enumerate}

\subsubsection{Related work to be considered}

\cite{CoMPNetX} -- They build a search tree using neural network guided growth. Generator of configurations + discriminator to assess the distance form the manifold used to project the configurations to the manifold + some constraint-adherence integrator to connect two configurations returned by the network. they consider manifold in configuration space only $c(\q)=0$. Learned using demonstration trajectories.

\cite{li2021mpcmpnet} -- They build a search tree using neural network guided growth. Generator is predicting the states, while the steering between them is done using \gls{mpc}. Discriminator is trained to predict the cost-to-go of a given state.
Learned using demonstration trajectories.

\cite{hung2022} -- They train \gls{vae} to encode the configurations and end-effector positions. In the inference they use gradient of the decoder to update the latent vector of the initial configuration towards the goal configuration. Collision classifier gradient used to avoid collisions. Unsupervised learning. Very vague dynamical feasibility of the movements, as they plan only sequence of configurations, and then show that their motions are super slow and do not violate any velocity nor acceleration constraints.

\cite{berenson2009manipulation} -- Sapling in the configuration space, with rejection or projection to satisfy configuration constraints. Does not consider velocity constraints, but can "somewhat" handle torque constraints by the rejection procedure, however, based on the \gls{rnea} calculated to maintain given configuration - quasi-static.

\cite{bordalba2018} -- Iteratively grows, using \gls{rrt}, the search tree of the configurations and velocities and the atlas of the local mappings between configuration space and constraint manifold, which is used to sample and connect nodes.
 
\cite{mukadam2018gpmp2} -- Gaussian Process based motion planning. They optimize the trajectory represented with a GP using factor graph formulation. They can impose constraints on the end-effector position, as well as the velocity and acceleration limits by introducing some priors on the GP, however including velocities and accelerations increase the size of the state, what slows down the optimization. I'm not sure if and how they optimize the duration of the movement.
\cite{dGPMP2} differentiable version of the GPMP2 -- ability to learn some hyper-parameters of GPMP2 from experience.

\cite{unsupervised_path_regression} -- They train neural network without any supervision how to plan short non-colliding NURBS paths between given initial and desired configuration. To learn how to avoid collisions they use SDF.
Quite similar idea to our one, but they plan paths only so do do not include velocity, acceleration limits, as well as end-effector constraints.

\cite{factor_graph_dynamics_optimization} -- Nonlinear optimization for dynamically constrained systems with the use of factor graph formalism. They seem to be able do what we do, but there is no information about the quality of the generated trajectories nor planning times.

\cite{factor_graph_dynamics_optimization_2} -- Looks like some other version of \cite{factor_graph_dynamics_optimization}. They added some experiments concerning minimum torque reaching task with Kuka Iiwa with no constraints on the end-effector, however, planning takes about 2s and they do not shared he code, so it is hard to compare with them on the same task.


\cite{learning_solution_manifold} -- They are training the 
latent variable model to generate the optimal "trajectory" based on the given latent variable, thus they are trying to capture the solution manifold and sample "trajectories" from it. They consider only a reaching task and limits on the joint positions, as they "trajectories" are represented by a sequence of configurations.
    
\subsubsection{Old derivations}

To solve this problem effectively, we rely on two key ideas. First, we consider only trajectories parametrized by a vector~$\vtheta$. Second, we apply a Lagrange relaxation technique \cite{bertsekas_largrange} to \eqref{eq:problem_formulation}, framing it as an unconstrained optimization of the following loss function:
\begin{equation}
    \Loss = \Loss + \lm^T\manifoldLoss,
\end{equation}
where $\Loss$ is our original task loss which describe the desired task, $\manifoldLoss$ is the vector of constraint manifold losses i.e. a losses that measure the violation of the defined constraints of the current trajectory, while $\lm$ is a vector of Lagrange multipliers. In most of the cases both the task loss $\Loss$ and individual manifold losses $\manifoldLoss^i$ will counteract each other, thus we would like to introduce an acceptable level of the constraint violation $\bLMi$ for each constraint. Therefore our constrained optimization problem can be framed as
\begin{align}
    \argmin_{\vtheta}  \quad  & \Loss \nonumber\\
    \text{s.t.}  \quad  & \manifoldLoss^i \leq \bLMi & \forall i, 0 \leq i < N + M
    \label{eq:constrained_opt_ours}
\end{align}
% \todo{add relaxed form of this?}
and relaxed to the following unconstrained form
\begin{equation}
    \label{eq:constrained_opt_ours_relaxed}
    \argmin_{\vtheta} \max_{\lm} \quad L(\vtheta, \lm)
\end{equation}
where
\begin{equation}
    L = \Loss + \lm^T \begin{bmatrix}\frac{\Loss_{\manifold_0}}{\bar{\Loss}_{\manifold_0}} & \frac{\Loss_{\manifold_1}}{\bar{\Loss}_{\manifold_1}} & \ldots & \frac{\Loss_{\manifold_{N+M-1}}}{\bar{\Loss}_{\manifold_{N+M-1}}} \end{bmatrix}^T - \sum_{i=0}^{N+M-1} \manifoldLoss^i.
\end{equation}


The most common approaches to solve \eqref{eq:constrained_opt_ours_relaxed} rely on calculating the gradients of the \eqref{eq:constrained_opt_ours_relaxed} w.r.t. to $\vtheta$ and $\lm$ and updating $\vtheta$ and $\lm$ using gradient descent and ascent respectively~\cite{lagrange_constraints}, however, we found updating $\lm$ according to this rule inefficient and therefore we propose a different update rule. \todo{Should we also mention here that we will take a gradient of $\Loss$ instead of $L$ to modify the parameters $\vtheta$?} Given that all $\manifoldLoss^i$ should be positive we propose a parametrization $\manifoldLoss^i \triangleq e^{\alpha_i}$ and introduce an update rule for $\alpha_i$ defined by
\begin{equation}
    \label{eq:alpha_update_rule}
    \Delta\alpha_i = \gamma \log\pare{\frac{\Loss_{\manifold_i}}{\bar{\Loss}_{\manifold_i}}},
\end{equation}
where $\gamma$ is an update step size. The rationale behind \eqref{eq:alpha_update_rule} stems from the analysis of the change of the loss value between $k$-th and $k+1$-th iterations i.e. let's define a complement of the $i$-th manifold loss element as $\cLMi \triangleq \Loss - \manifoldLoss^i$ and analyze how the $\alpha_i$ should change in order to achieve $\bLMi$ i.e.
\begin{equation}
   \cLMi + e^{\alpha_i} \manifoldLoss^i = \cLMi + e^{\alpha_i} \bLMi
\end{equation}
and assuming that the change of $\cLMi$ is small, what can be justified by a relatively small learning rate used in the neural network training, we get 
\begin{equation}
   e^{\alpha_i} \manifoldLoss^i = e^{\alpha_i} \bLMi \Rightarrow \alpha_i - \alpha_i = \log\pare{\frac{\manifoldLoss^i}{\bLMi}}
\end{equation}
and in order to smooth out the changes of $\alpha_i$ we introduce a scaling factor $\gamma$ and obtain \eqref{eq:alpha_update_rule}. 

\todo{Should I describe here the simplification that we have single alpha per constraint group?}

\subsubsection{The Manifold Loss}

Let $c(\q,\dq, \ddq)$ be a constraint function $c: \mathbb{R}^{3n}\to\mathbb{R}^m$, where $n$ is the number of generalized coordinates and $m$ is the number of constraints. Thus the function c can be written in vectorial form as:
\begin{equation}
    c(\q,\dq, \ddq) = \left[ c_0(\q,\dq, \ddq), \dots, c_i(\q,\dq, \ddq), \dots c_{m-1}(\q,\dq, \ddq) \right]^T.
\end{equation}
We define our constraint manifold as the 0-level curve of the constraint function $c(\q,\dq, \ddq)$
\begin{equation}
\manifold = \lbrace (\q, \dq, \ddq) \mid c(\q, \dq, \ddq) = 0\rbrace    
\end{equation}

We define our manifold loss as:
\begin{equation}
    \manifoldLoss = c(\q,\dq, \ddq)^Tc(\q,\dq, \ddq) = \sum_{i=0}^m c_i(\q,\dq, \ddq)^2 = \sum_{i=0}^m \manifoldLoss^i,
\end{equation}

In the following, we prove that we can express with this form both equality and inequality constraints. For equality constraints we have, trivially, that the $i$-th constraint will have the form:
\begin{equation}
    c_i(\q,\dq, \ddq) = 0
\end{equation}
For inequality constraints in the form $f(\cdot) \geq 0$, we introduce the slack variable $\slack$. Then we write the $j$-th constraint in the form:
\begin{equation}
     c_j(\q,\dq, \ddq, \slack) = f(\q,\dq, \ddq) - \slack^2 = 0
\end{equation}
Thus we have obtain 
\begin{align}
     \manifoldLoss^i(\q,\dq, \ddq, \slack) & = c_j(\q,\dq, \ddq, \slack)^2 = \left(f(\q,\dq, \ddq) - \slack^2\right)^2\\
          & = f(\q,\dq, \ddq)^2 - 2f(\q,\dq, \ddq)\slack^2 + \slack^4 
\end{align}
We now define our loss for inequality constraint as follows:
\begin{equation}
     \manifoldLoss^i(\q,\dq, \ddq) = \min_{\slack}\manifoldLoss^i(\q,\dq, \ddq, \slack)
\end{equation}
We can find the value that minimize $\manifoldLoss^i(\q,\dq, \ddq, \slack)$ by taking the derivative w.r.t. the slack variable at setting it to zero:
\begin{equation}
    \dfrac{d}{d\slack}\manifoldLoss^i(\q,\dq, \ddq, \slack) = -4f(\q,\dq, \ddq)\slack + 4\slack^3 = 0
\end{equation}
thus we obtain $\slack = 0 \vee \slack = \pm \sqrt{f(\q,\dq, \ddq)}$, where the second solution exists only for $f(\q,\dq, \ddq) > 0$. Plugging back the obtained stationary points in the solution, by basic reasoning of the obtained values and conditions, we obtain our inequality loss
\begin{equation}
     \manifoldLoss^i(\q,\dq, \ddq) = \begin{cases} 
     0 & f(\q,\dq, \ddq) > 0 \\
     f(\q,\dq, \ddq)^2 & \textbf{otherwise}
     \end{cases}
\end{equation}
This loss can be computed compactly, in an equivalent form as
\begin{equation}
     \manifoldLoss^i(\q,\dq, \ddq) = \left(\min \left(f(\q,\dq, \ddq), 0\right)\right)^2
\end{equation}
which is continuous and differentiable everywhere: notice that in 0, the derivative is 0.
We formulate strict inequality constraints by adding a small offset $\epsilon>0$ to the original constraint i.e., $f'(\q,\dq,\ddq)=f(\q,\dq,\ddq)-\epsilon$. Indeed, due to practical computational reasons, this kind of formulation is indistinguishable from a mathematically accurate one.

Finally, we remark that a dynamic constraint i.e., a constraint depending on the torque $\torque$, can be described with the same framework by considering the relationship $\torque=\inversedynamics(\q, \dq, \ddq)$, where $\inversedynamics$ are the inverse dynamics of the system.


==> cover_note.tex <==
Our paper presents a novel approach to the topic of learning to plan. We focus on kinodynamic motion planning tasks with constraints imposed on the robot's joint velocities, acceleration, and torques, as well as, the robot's movement in the task space i.e. collision avoidance and maintaining the end-effector on some predefined manifold.
This paper is accompanied by the video attachment, code with datasets (https://github.com/pkicki/cnp-b), and website  (https://sites.google.com/view/constrained-neural-planning) containing additional material, including the full recordings of the robotics experiments.
